Spherical means with centers on a hyperplane in even dimensions

Given a real valued function on R^n we study the problem of recovering the function from its spherical means over spheres centered on a hyperplane. An old paper of Bukhgeim and Kardakov derived an inversion formula for the odd n case with great simplicity and economy. We apply their method to derive an inversion formula for the even n case. A feature of our inversion formula, for the even n case, is that it does not require the Fourier transform of the mean values or the use of the Hilbert transform, unlike the previously known inversion formulas for the even n case. Along the way, we extend the isometry identity of Bukhgeim and Kardakov for odd n, for solutions of the wave equation, to the even n case.

==> integral-calculations.tex <==
\section{Some integral calculations}
Let $w=a+ib$ with $a,b$ real, $a>0$ and let $\tau \in \R$. We have (the absolutely convergent integral)
\begin{align*}
I := \int_\R e^{-w t^2} e^{-it\tau} \, dt
& = \int_\R e^{ -w (t^2 +it \tau/w)} \, dt
=  e^{-\tau^2/(4w)} \int_\R e^{-w (t + i \tau/(2w))^2} \, dt
= e^{-\tau^2/(4w)} \int_{\Gamma} e^{-w z^2} \, dz
\end{align*}
where $\Gamma$ is the horizontal line $\Im z = \Im w^{-1}$. Since the last integral is convergent and so is $\int_\R e^{-w t^2} \, dt$ and
$\lim_{M \rightarrow \infty} |e^{-wz^2}| =0$ uniformly on the segments
$ \Re z = \pm M$, $ 0 \leq \Im z \leq c$, we have
%
\[
I = \int_\R e^{-w t^2}\, dt = 2\int_0^\infty e^{-w t^2} \, dt
= \frac{2}{ \sqrt{w}}\int_{\Sigma} e^{-z^2} \, dz
\]
where $\Sigma$ is the ray $z=t \sqrt{w}$, $t \geq 0$. Using the decay properties of $e^{-z^2}$ one can show that
\[
I = \frac{2}{\sqrt{w}} \int_0^\infty e^{-t^2} \, dt = \frac{\sqrt{\pi}}{\sqrt{w}}.
\]

Also, again using the standard complex analysis techniques, if $\Sigma$ is the ray $tw$, $t \geq 0$, then we have
\begin{align*}
\int_0^\infty \frac{e^{-wt}}{\sqrt{t}} \, dt
= \frac{1}{ \sqrt{w}} \int_\Sigma \frac{ e^{-z}}{\sqrt{z}} \, dz
= \frac{1}{\sqrt{w}} \int_0^\infty \frac{e^{-t}}{\sqrt{t}} \, dt
=\frac{ \Gamma(1/2)}{ \sqrt{w}} = \frac{ \sqrt{\pi}}{ \sqrt{w}}.
\end{align*}
% 
